Enhancing Deep Knowledge Tracing with Auxiliary Tasks

Knowledge tracing (KT) is the problem of predicting students' future performance based on their historical interactions with intelligent tutoring systems. Recent studies have applied multiple types of deep neural networks to solve the KT problem. However, there are two important factors in real-world educational data that are not well represented. First, most existing works augment input representations with the co-occurrence matrix of questions and knowledge components\footnote{\label{ft:kc}A KC is a generalization of everyday terms like concept, principle, fact, or skill.} (KCs) but fail to explicitly integrate such intrinsic relations into the final response prediction task. Second, the individualized historical performance of students has not been well captured. In this paper, we proposed \emph{AT-DKT} to improve the prediction performance of the original deep knowledge tracing model with two auxiliary learning tasks, i.e., \emph{question tagging (QT) prediction task} and \emph{individualized prior knowledge (IK) prediction task}. Specifically, the QT task helps learn better question representations by predicting whether questions contain specific KCs. The IK task captures students' global historical performance by progressively predicting student-level prior knowledge that is hidden in students' historical learning interactions. We conduct comprehensive experiments on three real-world educational datasets and compare the proposed approach to both deep sequential KT models and non-sequential models. Experimental results show that \emph{AT-DKT} outperforms all sequential models with more than 0.9\% improvements of AUC for all datasets, and is almost the second best compared to non-sequential models. Furthermore, we conduct both ablation studies and quantitative analysis to show the effectiveness of auxiliary tasks and the superior prediction outcomes of \emph{AT-DKT}.

==> limitation.tex <==
Most existing DLKT research relies on the binary response assumption and existing publicly available datasets only contain the binary labels, i.e., correct or incorrect. We believe this is because the binary valued data is (sort of) the most objective assessment labels that can be easily collected from either the online learning platforms or the offline classrooms on a large scale. However, we deeply believe that having more fine-grained student assessment labels beyond the binary value of correct and incorrect would push the boundary of this research field. Some research works such as option tracing \cite{ghosh2021option} aim to extend existing KT methods beyond correctness prediction to the task of predicting the exact option students select in multiple choice questions. This only works for multiple choice questions and it generalizes the traditional KT prediction from binary classification to the multi-class classification settings. The proposed AT-DKT model is well-modularized and different loss functions or evaluation metrics can be easily added. Hence, it is flexible to extend the existing benchmark to non-binary prediction settings such as multi-class classification or real-valued regression problems. 
